Population-based Optimization for Kinetic Parameter Identification in Glycolytic Pathway in Saccharomyces cerevisiae

Models in systems biology are mathematical descriptions of biological processes that are used to answer questions and gain a better understanding of biological phenomena. Dynamic models represent the network through rates of the production and consumption for the individual species. The ordinary differential equations that describe rates of the reactions in the model include a set of parameters. The parameters are important quantities to understand and analyze biological systems. Moreover, the perturbation of the kinetic parameters are correlated with upregulation of the system by cell-intrinsic and cell-extrinsic factors, including mutations and the environment changes. Here, we aim at using well-established models of biological pathways to identify parameter values and point their potential perturbation/deviation. We present our population-based optimization framework that is able to identify kinetic parameters in the dynamic model based on only input and output data (i.e., timecourses of selected metabolites). Our approach can deal with the identification of the non-measurable parameters as well as with discovering deviation of the parameters. We present our proposed optimization framework on the example of the well-studied glycolytic pathway in Saccharomyces cerevisiae.

==> original_content.tex <==
The Elsevier cas-dc class is based on the
% standard article class and supports almost all of the functionality of
% that class. In addition, it features commands and options to format the
% \begin{itemize} \item document style \item baselineskip \item front
% matter \item keywords and MSC codes \item theorems, definitions and
% proofs \item lables of enumerations \item citation style and labeling.
% \end{itemize}

% This class depends on the following packages
% for its proper functioning:

% \begin{enumerate}
% \itemsep=0pt
% \item {natbib.sty} for citation processing;
% \item {geometry.sty} for margin settings;
% \item {fleqn.clo} for left aligned equations;
% \item {graphicx.sty} for graphics inclusion;
% \item {hyperref.sty} optional packages if hyperlinking is
%   required in the document;
% \end{enumerate}  

% All the above packages are part of any
% standard \LaTeX{} installation.
% Therefore, the users need not be
% bothered about downloading any extra packages.

% \section{Installation}

% The package is available at author resources page at Elsevier
% (\url{http://www.elsevier.com/locate/latex}).
% The class may be moved or copied to a place, usually,\linebreak
% \verb+$TEXMF/tex/latex/elsevier/+, %$%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% or a folder which will be read                   
% by \LaTeX{} during document compilation.  The \TeX{} file
% database needs updation after moving/copying class file.  Usually,
% we use commands like \verb+mktexlsr+ or \verb+texhash+ depending
% upon the distribution and operating system.

% \section{Front matter}

% The author names and affiliations could be formatted in two ways:
% \begin{enumerate}[(1)]
% \item Group the authors per affiliation.
% \item Use footnotes to indicate the affiliations.
% \end{enumerate}
% See the front matter of this document for examples. 
% You are recommended to conform your choice to the journal you 
% are submitting to.

% \section{Bibliography styles}

% There are various bibliography styles available. You can select the
% style of your choice in the preamble of this document. These styles are
% Elsevier styles based on standard styles like Harvard and Vancouver.
% Please use Bib\TeX\ to generate your bibliography and include DOIs
% whenever available.

% Here are two sample references: 
% \cite{Fortunato2010}
% \cite{Fortunato2010,NewmanGirvan2004}
% \cite{Fortunato2010,Vehlowetal2013}

% \section{Floats}
% {Figures} may be included using the command,\linebreak 
% \verb+\includegraphics+ in
% combination with or without its several options to further control
% graphic. \verb+\includegraphics+ is provided by {graphic[s,x].sty}
% which is part of any standard \LaTeX{} distribution.
% {graphicx.sty} is loaded by default. \LaTeX{} accepts figures in
% the postscript format while pdf\LaTeX{} accepts {*.pdf},
% {*.mps} (metapost), {*.jpg} and {*.png} formats. 
% pdf\LaTeX{} does not accept graphic files in the postscript format. 

% \begin{figure}
% 	\centering
% 		\includegraphics[scale=.75]{figs/Fig1.pdf}
% 	\caption{The evanescent light - $1S$ quadrupole coupling
% 	($g_{1,l}$) scaled to the bulk exciton-photon coupling
% 	($g_{1,2}$). The size parameter $kr_{0}$ is denoted as $x$ and
% 	the \PMS is placed directly on the cuprous oxide sample ($\delta
% 	r=0$, See also Table \protect\ref{tbl1}).}
% 	\label{FIG:1}
% \end{figure}


% The \verb+table+ environment is handy for marking up tabular
% material. If users want to use {multirow.sty},
% {array.sty}, etc., to fine control/enhance the tables, they
% are welcome to load any package of their choice and
% {cas-dc.cls} will work in combination with all loaded
% packages.

% \begin{table}[width=.9\linewidth,cols=4,pos=h]
% \caption{This is a test caption. This is a test caption. This is a test
% caption. This is a test caption.}\label{tbl1}
% \begin{tabular*}{\tblwidth}{@{} LLLL@{} }
% \toprule
% Col 1 & Col 2 & Col 3 & Col4\\
% \midrule
% 12345 & 12345 & 123 & 12345 \\
% 12345 & 12345 & 123 & 12345 \\
% 12345 & 12345 & 123 & 12345 \\
% 12345 & 12345 & 123 & 12345 \\
% 12345 & 12345 & 123 & 12345 \\
% \bottomrule
% \end{tabular*}
% \end{table}

% \section[Theorem and ...]{Theorem and theorem like environments}

% {cas-dc.cls} provides a few shortcuts to format theorems and
% theorem-like environments with ease. In all commands the options that
% are used with the \verb+\newtheorem+ command will work exactly in the same
% manner. {cas-dc.cls} provides three commands to format theorem or
% theorem-like environments: 

% \begin{verbatim}
%  \newtheorem{theorem}{Theorem}
%  \newtheorem{lemma}[theorem]{Lemma}
%  \newdefinition{rmk}{Remark}
%  \newproof{pf}{Proof}
%  \newproof{pot}{Proof of Theorem \ref{thm2}}
% \end{verbatim}


% The \verb+\newtheorem+ command formats a
% theorem in \LaTeX's default style with italicized font, bold font
% for theorem heading and theorem number at the right hand side of the
% theorem heading.  It also optionally accepts an argument which
% will be printed as an extra heading in parentheses. 

% \begin{verbatim}
%   \begin{theorem} 
%   For system (8), consensus can be achieved with 
%   $\|T_{\omega z}$ ...
%      \begin{eqnarray}\label{10}
%      ....
%      \end{eqnarray}
%   \end{theorem}
% \end{verbatim}  


% \newtheorem{theorem}{Theorem}

% \begin{theorem}
% For system (8), consensus can be achieved with 
% $\|T_{\omega z}$ ...
% \begin{eqnarray}\label{10}
% ....
% \end{eqnarray}
% \end{theorem}

% The \verb+\newdefinition+ command is the same in
% all respects as its \verb+\newtheorem+ counterpart except that
% the font shape is roman instead of italic.  Both
% \verb+\newdefinition+ and \verb+\newtheorem+ commands
% automatically define counters for the environments defined.

% The \verb+\newproof+ command defines proof environments with
% upright font shape.  No counters are defined. 


% \section[Enumerated ...]{Enumerated and Itemized Lists}
% {cas-dc.cls} provides an extended list processing macros
% which makes the usage a bit more user friendly than the default
% \LaTeX{} list macros.   With an optional argument to the
% \verb+\begin{enumerate}+ command, you can change the list counter
% type and its attributes.

% \begin{verbatim}
%  \begin{enumerate}[1.]
%  \item The enumerate environment starts with an optional
%   argument `1.', so that the item counter will be suffixed
%   by a period.
%  \item You can use `a)' for alphabetical counter and '(i)' 
%   for roman counter.
%   \begin{enumerate}[a)]
%     \item Another level of list with alphabetical counter.
%     \item One more item before we start another.
%     \item One more item before we start another.
%     \item One more item before we start another.
%     \item One more item before we start another.
% \end{verbatim}

% Further, the enhanced list environment allows one to prefix a
% string like `step' to all the item numbers.  

% \begin{verbatim}
%  \begin{enumerate}[Step 1.]
%   \item This is the first step of the example list.
%   \item Obviously this is the second step.
%   \item The final step to wind up this example.
%  \end{enumerate}
% \end{verbatim}

% \section{Cross-references}
% In electronic publications, articles may be internally
% hyperlinked. Hyperlinks are generated from proper
% cross-references in the article.  For example, the words
% \textcolor{black!80}{Fig.~1} will never be more than simple text,
% whereas the proper cross-reference \verb+\ref{tiger}+ may be
% turned into a hyperlink to the figure itself:
% \textcolor{blue}{Fig.~1}.  In the same way,
% the words \textcolor{blue}{Ref.~[1]} will fail to turn into a
% hyperlink; the proper cross-reference is \verb+\cite{Knuth96}+.
% Cross-referencing is possible in \LaTeX{} for sections,
% subsections, formulae, figures, tables, and literature
% references.

% \section{Bibliography}

% Two bibliographic style files (\verb+*.bst+) are provided ---
% {model1-num-names.bst} and {model2-names.bst} --- the first one can be
% used for the numbered scheme. This can also be used for the numbered
% with new options of {natbib.sty}. The second one is for the author year
% scheme. When  you use model2-names.bst, the citation commands will be
% like \verb+\citep+,  \verb+\citet+, \verb+\citealt+ etc. However when
% you use model1-num-names.bst, you may use only \verb+\cite+ command.

% \verb+thebibliography+ environment.  Each reference is a\linebreak
% \verb+\bibitem+ and each \verb+\bibitem+ is identified by a label,
% by which it can be cited in the text:

% \noindent In connection with cross-referencing and
% possible future hyperlinking it is not a good idea to collect
% more that one literature item in one \verb+\bibitem+.  The
% so-called Harvard or author-year style of referencing is enabled
% by the \LaTeX{} package {natbib}. With this package the
% literature can be cited as follows:

% \begin{enumerate}[\textbullet]
% \item Parenthetical: \verb+\citep{WB96}+ produces (Wettig \& Brown, 1996).
% \item Textual: \verb+\citet{ESG96}+ produces Elson et al. (1996).
% \item An affix and part of a reference:\break
% \verb+\citep[e.g.][Ch. 2]{Gea97}+ produces (e.g. Governato et
% al., 1997, Ch. 2).
% \end{enumerate}

% In the numbered scheme of citation, \verb+\cite{<label>}+ is used,
% since \verb+\citep+ or \verb+\citet+ has no relevance in the numbered
% scheme.  {natbib} package is loaded by {cas-dc} with
% \verb+numbers+ as default option.  You can change this to author-year
% or harvard scheme by adding option \verb+authoryear+ in the class
% loading command.  If you want to use more options of the {natbib}
% package, you can do so with the \verb+\biboptions+ command.  For
% details of various options of the {natbib} package, please take a
% look at the {natbib} documentation, which is part of any standard
% \LaTeX{} installation.

% \appendix
% \section{My Appendix}
% Appendix sections are coded under \verb+\appendix+.

% \verb+\printcredits+ command is used after appendix sections to list 
% author credit taxonomy contribution roles tagged using \verb+\credit+ 
% in frontmatter.
